A bibliometric analysis and scoping study to identify English-language perspectives on slums

Slums, informal settlements, and deprived areas are urban regions characterized by poverty. According to the United Nations, over one billion people reside in these areas, and this number is projected to increase. Additionally, these settlements are integral components of urban systems. We conducted a bibliometrical analysis and scoping study using the Web of Science Database to explore various perspectives on urban poverty, searching for scientific publications on the topic and providing details on the countries where the studies were conducted. Based on 3947 publications, we identify the extent to which domestic research organizations participate in studying urban poverty and which categories of science they investigate, including life sciences \& biomedicine, social sciences, technology, physical sciences, and arts & humanities. Thereby, we find that research on slums is often limited to specific countries, e.g. India, South Africa, Kenya, or Brazil. This focus is not necessarily correlated with the number of people living in slums. The scientific discourse is up to now predominantly shaped by medical and social sciences with few studies addressing technological questions. Finally, our analysis identifies several possible future directions for research on slums.

==> additonal_information.tex <==
\begin{itemize}
    
    \item Die Tatsache, dass Südafrika besonders viele Studien pro Slumbewohner aufweist gilt es kritisch zu beleuchten: Der Begriff "township", der im Zusammenhang mit südafrikanischen Länder häufig für informelle urbane Siedlungen verwendet wird, ist weiter gefasst als der Begriff Slums. [Stimmt das? Dass ist zumindest mein Eindruck beim sichten der Literatur] Die hohe Zahl an Studien in Südafrika ist also nur bedingt mit den Werten für Studien pro Einwohner in Slums in anderen Ländern vergleichbar.
    \item Auf grund der manchmal kleinen absoluten Zahl an Publikationen für gewisse Filterkriterien, haben mache Aussagen (insebsondere relative Analysen) eine geringe Aussagekraft.
\end{itemize}

\section{Additional Stuff}

\begin{itemize}
    \item Tab.~\ref{tab:InstitutionsWithMostCitations_Absolute}: Ohne Postprocessing der Forschungsinstitutionen werden im Datensatz 3141 verschiedene Institutionen gefunden. Statt unter all diesen Institutionen nach Dublikaten zu suchen (z.B. 'aga kahn univ', 'aga khan univ', 'aga khan univ \& hosp', 'aga khan univ hosp'). Habe ich mir die 21 Insitutionen mit a) den meisten kumulativen Zitationen, b) den meisten Publikationen und c) den meisten Zitationen bezogen auf die Anzahl an Zitationen angeschaut. Für diese Insitutionen habe ich nach Dublikaten gesucht und die Datenerfassung diesbezüglich korrigiert. Anschließend habe ich die Top-Institutionen ermittelt.
    \item Tab.~\ref{tab:InstitutionsWithMostCitations_Absolute}: University London, und University Texas könnte man als Universitätsverbund in die Liste aufnahmen, dann würden sich die Ergebnisse sicher ändern
\end{itemize}



%OLD Introduction
The unequal distribution of resources and living space has been described as a characteristic of cities since ancient times \cite{Fuks.1977}. While some of the inhabitants have adequate access to infrastructures of transportation, health care or water supply, this access is often denied to other parts of the urban population leading to a polar division. %This unequal distribution can show different manifestations in different regions of the world.
% This introduction to me seems like we are motivating writing about unequal distribution and access to infrastructure etc, not about research on slums. I think we could open with a paragraph that directly links to our research subject in order to put the interested reader on track immediately

This can be observed in a consistent manner across  many countries of the Global South, where so-called \textit{informal settlements} or \textit{slums} characterize the urban landscape \cite{Mahabir.2016}. While informal settlements are characterized primarily by their non-formal settlement status, slums are defined by the United Nations as areas or households in which at least one of the following five criteria is met: (i) inadequate access to safe water, (ii) inadequate access to sanitation, (iii) poor structural quality of housing, (iv) overcrowding or (v) insecure residential status. 

According to the World Bank, more than one billion people live in slums. These populations are distributed across the globe as shown in Figure \ref{fig:slumpopu}. Most slum residents, according to these numbers live in India (237 Mio.), Nigeria (52 Mio.), and Indonesia (30 Mio.). The absolute number of people can be seen as an indicator of the importance of doing research in the respective country. Kanai et al. \cite{Kanai.2018} have done a similar study for urban areas. %Similar to what and in what way?

The informal character of these settlements means that they are often referred to as \textit{invisible} in research. %references? 
They are also often the blind spots of local administration, which can be illustrated particularly impressively by the fact that in India a distinction is made between \textit{notified} and \textit{non-notified} slums \cite{Nolan.2018}.

At the same time, this invisibility means that the inhabitants of these forms of settlement are often excluded from urban provisions, services and infrastructures, as mentioned above, which  can in turn often lead to health disadvantages (e.g. \cite{Garenne.2010, Scott.2017}), both physical and psychological.  This can be easily understood from the example of sanitation and the connection between its non-existence and infectious diseases \cite{Ezeh.2017}.

The multidimensional deprivation of the inhabitants of informal settlements is one reason why, since the early 2000s, this form of settlement has increasingly become the focal point on the political agenda, manifested in the Millennium and Sustainable Development Goals (here especially and explicitly in SDG 11.1, where a reduction of population living in slums is aimed for), pop culture, as evidenced by Oscar-winning movies such as \textit{City of God} or \textit{Slumdog Millionaire} \cite{Roy.2011} and scientific research. 

It was pointed out that research on slums is characterized by discourses of power, which is evident, for example, in the negative connotation of the word \textit{slum}, often not used as a self-designation but imposed on the settlement areas and their inhabitants from the outside. Slum dwellers are often the object of analysis and rarely enter the research discourse as participating subjects. These problems have already been raised and discussed thoroughly \cite{GILBERT.2007,Roy.2011,Mayne.2017}. In order to obtain a more comprehensive perspective on urban poverty, the \textit{Domains of deprivation framework} has therefore been developed in recent years \cite{Abascal.2022}. This seeks a more comprehensive understanding of deprivation and also refers to settlements as \textit{deprived areas} rather than slums. Although the term \textit{deprived areas} addresses the question of disadvantage more comprehensively, we will continue to use the term slums in the following, as it has dominated research in recent decades.  %These issues are particularly insistent in the study of social contexts, as these are always associated with constellations of power, explained by the concept of epistemic violence. 

The perspective on a certain phenomenon shapes the outcome of the research on it and especially in the last years, a number of publications have pointed out that in the research context there are strong differences in the distribution of race, ethnicity \cite{Hrabowski.2020} and gender \cite{Huang.2020} of the researchers. Looking at different perspectives of researchers and diversity in (economic) geography \cite{Rosenman.2020}, Rosenman et al. show that certain groups, like women, are underrepresented in the scientific discourse.

This phenomenon can also be applied at different levels to settlements of deprivation/ slums/ informal settlements etc. The focus of media, exemplary projects or scientific publications is often on big popular slums like Orangi in Karachi (Pakistan), Dharavi in Mumbai (India), Kibera in Nairobi (Kenya) or Paraisopolis in Sao Paulo (Brazil), although the majority of the dwellers seem to live in smaller settlements \cite{Friesen.2018}. It was also shown that medical studies are mainly distributed in certain countries and thereby in specific cities, while other countries are neglected \cite{Friesen.2020}.

These observations highlight the relevance to reflect on research itself. 
Hence, we perfom a bibliometric analysis to answer the following questions:

Which countries and regions were primarily investigated in the last years? With which organizations are the researchers affiliated with and where are these organizations based? How has the amount of studies on slums in specific countries developed over time? Which topics/themes stand in the foreground?  How is the knowledge of slums spatially distributed, and, by extension, how representative is the research on slums?

Our goal is not to provide a literature review on current developments in slum research. For this, we refer to studies that have already been conducted for example about the state of research on slum dweller health \cite{Ezeh.2017}, dwelling classification and modeling \cite{Mahabir.2016, Kuffer.2016}, population estimates \cite{Thomson.2021}, economics \cite{Marx.2013} and many others. Instead, we believe that quantiative analysis (similar to Biswas et al. \cite{Biswas.2021}) can provide valuable insights into the geographic and thematic distribution of research on urban deprivation.

